Near-Optimal Representation Learning for Hierarchical Reinforcement Learning

We study the problem of representation learning in goal-conditioned hierarchical reinforcement learning. In such hierarchical structures, a higher-level controller solves tasks by iteratively communicating goals which a lower-level policy is trained to reach. Accordingly, the choice of representation -- the mapping of observation space to goal space -- is crucial. To study this problem, we develop a notion of sub-optimality of a representation, defined in terms of expected reward of the optimal hierarchical policy using this representation. We derive expressions which bound the sub-optimality and show how these expressions can be translated to representation learning objectives which may be optimized in practice. Results on a number of difficult continuous-control tasks show that our approach to representation learning yields qualitatively better representations as well as quantitatively better hierarchical policies, compared to existing methods (see videos at https://sites.google.com/view/representation-hrl).

==> notation.tex <==

\begin{table}[t]
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
         Symbol & Type & Definition \\ \hline
         $\gM$ & MDP & MDP. \\ 
         $S$ & Set & State space. \\ 
         $A$ & Set & Action space (on $\gM$). \\ 
         $R$ & $S\to\R$ & Reward (on $\gM$). \\
         $R_{max}$ & $\R$ & $\sup_{S} |R(s)|$. \\
         $\gamma$ & $\R$ & Discount. \\
         $\pilo$ & Policy & Lower-level policy. \\
         $\pihi$ & Policy & Higher-level policy. \\
         $c$ & $\mathbb{N}$ & Temporal abstraction.  Every $c$ steps, $\pihi$ chooses new goal. \\
         $k$ & $\mathbb{N}$ & Index into $[0, c-1]$. \\
         $d$ & $\mathbb{N}$ & Goal dimension.  State representation dimension. \\
         $\tA$ & $\R^d$ & Goal space.  High-level action space. \\
        $\ta$ & $\tA$ & Goal. \\
        $f$ & $S\to \tA$ & State representation function. \\
        $D$ & $\R^d\times\R^d\to\R$ & Distance function in goal space. \\
        $\Z(s,g)$ & $S\times\tA\to\Pi$ & Mapping of state-goal to lower-level behavior policy. \\ 
        $\Pi$ & Set of policies & Set of candidate $c$-step lower-level behavior policies. \\
        $\pi$ & $\Pi$ & Lower-level behavior policy. Element of $\Pi$. \\
        $P_\pi(s_{t+k}|s_t)$ & Probability & Distribution of states $k$ steps in future when following $\pi$ from $s_t$. \\
        $\pihi^*$ & Policy & Optimal max reward higher-level policy using $\Z$. \\
        $\pihier^*$ & Policy & Optimal max reward hierarchical policy using $\Z$. \\
        $\pihi^{**}$ & Policy & Optimal max reward higher-level policy agnostic to $\Z$. \\ %with ability to sample any lower-level $\pi\in\Pi$. \\
        $\pistar$ & Policy & Optimal max reward hierarchical policy agnostic to $\Z$. \\
        $\subopt(\Z)$ & $\R$ & Sub-optimality of learning a hierarchical policy using $\Z$. \\ % compared to optimal hierarchical policy agnostic to $\Z$. \\
        $\Y(s,\pi)$ & $S\times\Pi\to\tA$ & Inverse goal model with respect to $\Z$. \\
        $K(s_{t+k}|s_t,\pi)$ & Probability & Approximate dynamics model based on $f,\Y$. \\
        $\rho(s)$ & Probability & Prior over $S$.  In practice, the replay buffer distribution. \\
        $w_k$ & $\R$ & Weights, $w_k=1$ for $k<c$ and $w_k=(1-\gamma)^{-1}$ for $k=c$. \\
        $\Wbar$ & $\R$ & Discounted sum of weights, $\sum_{k=1}^c \gamma^{k-1}w_k$. \\
        $\ftheta$ & $S\to\R^d$ & Parameterized state representation function. \\
        $\Ytheta$ & $S\times\Pi\to\tA$ & Parameterized version of $\Y$. \\
        $\Ktheta(s_{t+k}|s_t,\pi)$ & Probability & $K$ based on parameterized versions of $f, \Y$. \\
        $\Etheta(s',s,\pi)$ & $\R$ & $\exp(-D(\ftheta(s'),\Ytheta(s,\pi)))$  \\
        $J(\theta)$ & Objective & Representation learning objective. \\
        $J(\theta,s_t,\pi)$ & Objective & Representation learning objective for specific $s_t,\pi$. \\
        \hline
    \end{tabular}
    \caption{Notation used in this paper with corresponding abbreviated definitions.}
    \label{tab:my_label}
\end{table}
